Blockchain-Based, Confidentiality-Preserving Orchestration of Collaborative Workflows

Business process collaboration between independent parties can be challenging, especially if the participants do not have complete trust in each other. Tracking actions and enforcing the activity authorizations of participants via blockchain-hosted smart contracts is an emerging solution to this lack of trust, with most state-of-the-art approaches generating the orchestrating smart contract logic from BPMN models. However, as a significant drawback in comparison to centralized business process orchestration, smart contract state typically leaks potentially sensitive information about the state of the collaboration. We describe a novel approach where the process manager smart contract only stores cryptographic commitments to the state and checks zero-knowledge proofs on update proposals. We cover a representative subset of BPMN, support message passing commitments between participants and provide an open-source end-to-end implementation. Under our approach, no party external to the collaboration can gain trustable knowledge of the current state of a process instance (barring collusion with a participant), even if it has full access to the blockchain history.

==> content/DnO.tex <==
\section{Choosing a distributed ledger}
The state manager smart contract can run on two different distributed ledgers: 
\begin{enumerate}
    \item Ethereum (or other EVM-compatible ledgers)
    \item Hyperledger Fabric
\end{enumerate}
The verifier part of the smart contract for Ethereum is exported from ZoKrates. For Hyperledger Fabric We used the Zokrates fabric verifier we designed.

==> content/algorithm/statecheck_algo.tex <==
\begin{algorithm}[!h]
\caption{Proving that a state vector update is valid}\label{pseudo_code_valid}
\begin{algorithmic}[!h]
\Procedure{StateChange}{}
\State $v_{curr} \gets \text{Currnent state vector}$
\State $v_{next} \gets \text{New state vector}$
\State $A \gets [\textit{nothing};3] $
\For{$i\textbf{ in }0..\textit{len}(T)$}
\State \textbf{assert} $v_{curr}[i] <= 2$
\State \textbf{assert} $v_{next}[i] <= 2$
\EndFor
%\State pos $\gets 0$
\State \textit{changeCount} $\gets 0$
\For{$i\textbf{ in } 0..\textit{len}(T)$}
\If{$v_{next} == v_{curr}$} \textbf{continue}
\ElsIf{$v_{curr} == 1 \textbf{ and } v_{next} == 2$} 
\State $A[\textit{changeCount}] \gets [-1, i]$
\ElsIf{$v_{curr} == 0 \textbf{ and } v_{next} == 1$} 
\State $A[\textit{changeCount}] \gets [1, i]$
\Else
\State $A[\textit{changeCount}] \gets [-1, -1]$
\EndIf

\State $\textit{changeCount} \gets \textit{changeCount}+1$
\EndFor

%------- CONSTRUCT A END -------
\State \textbf{assert } \textit{changeCount} $\leq 3$
\If{\textit{changeCount} $== 0$}
\State \textbf{return true}
\EndIf
\State \textit{result} $\gets \textbf{false}$
\For{$i\textbf{ in } 0..W$}
\State \textit{allPairMatch} $\gets \textbf{true}$
\For{$j\textbf{ in } 0..3$}
\State \textit{pariFound} $\gets \textbf{false}$
\For{$k\textbf{ in } 0..3$}
\If{$A[k][0] == P[i][j][0] \textbf{ and } A[k][1] == P[i][j][1]$}
\State \textit{pariFound} $\gets \textbf{true}$
\EndIf
\EndFor
\If{$!$\textit{pariFound}}
\State \textit{allPairMatch} $\gets \textbf{false}$
\State \textbf{continue}
\EndIf
\EndFor
\If{$\textit{allPairMatch}$}
\State \textit{result}$\gets\textbf{ true}$
\EndIf
\EndFor
%------- COMPARE P END -------
\State \textit{// Testing for parallel gateway ends}
\If{\textit{changeCount} $== 1$}
\State \textit{ParallelTest}($A$)
\EndIf


%------- PARALLEL TEST --------
%------- END -------
\State \textbf{return} \textit{result}
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> content/testing.tex <==
\section{Testing}
To make sure this method of executing business processes is correct, We propose a few ways of challenging it.
\subsection{Test cases}
Our first method of testing our approach is by defining test cases and seeing if they can be used in our tool.
\subsubsection{Simple \& corner cases}
These test cases were designed to ensure that every supported element works. We also wanted to know how the program reacts to corner cases where the model syntax is correct but the semantics are questionable.

\paragraph{Kép kell ide?}

\subsubsection{Representative test}
As a Representative test, We wanted to use a complex, real-world example BPMN model. The goal is to see how the program reacts to more oversized state objects (e.g., more executable events, messages, etc.).

\paragraph{Kép kell ide?}

\subsubsection{Testing framework}
\label{testing_frame}
To run these tests We designed a testing framework. This framework can run individual test scenarios (i.g. separate steps) and run them as a batch.

The framework also has a GUI and CLI interface. The GUI can be accessed from WFGUI. The CLI interface is designed to work without user interaction. This makes it easy to integrate as a CI/CD pipeline.

\subsection{Future ideas for testing}
\label{more_tests}
An apparent insufficiency of the current approach is that it is not formally proven that the accepted language of the zkWF program conforms to formal specifications of BPMN model and execution semantics. 

This will be certainly a worthwhile area of future research. In addition to classic approaches, in this specific context, due to the relative simplicity of the involved components, it seems to be feasible to create a joint executable model of the smart contract, the prover, the communication protocol and lastly, an executable specification of BPMN semantics. This approach may be feasible even in the form of direct bytecode level model checking of an imperative language as Java (using, e.g., Java PathFinder for analysis). Then, operational semantics conformance can become checkable at least on a model-by-model basis.

==> content/tikz-figure/overview.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}[font=\sffamily,line width=0.03cm,line width=0.02cm, scale=0.70,every node/.style={scale=0.70}]
            
        \node[event] (start1) {};
        \node[task,right=0.5cm of start1,fill=green!30!white] (act) {\tiny A};
        \draw[-{Stealth[inset=0pt]}] (start1) -- (act);
	    \node[intermediate event,right=0.5cm of act,fill=green!30!white] (imt) {\tiny \faEnvelope};
	    \draw[-{Stealth[inset=0pt]}] (act) -- (imt);
	    \node[end event,right=0.5cm of imt](end1){};
	    \draw[-{Stealth[inset=0pt]}] (imt) -- (end1);
	    \node[minimum width=6.5cm,minimum height=2cm,draw,rectangle,fit=(imt) (act) (start1) (end1)](b){};
        \node[rotate=90,draw,rectangle,left=0.2cm of b,xshift=1cm,yshift=-\pgflinewidth*4,minimum width=2cm] (p){\tiny Participant 1};
        
        \node[intermediate event,below=1.5cm of imt,fill=orange!50!white] (imc) {\tiny\faEnvelope[regular]};
        \node[task,left=0.5cm of imc,fill=green!30!white] (act2) {\tiny B};
        \draw[-{Stealth[inset=0pt]}] (act2) -- (imc);
        \node[event,left=0.5cm of act2] (start2) {};
        \draw[-{Stealth[inset=0pt]}] (start2) -- (act2);
	    \node[end event,right=0.5cm of imc](end2){};
	    \draw[-{Stealth[inset=0pt]}] (imc) -- (end2);
	    \node[minimum width=6.5cm,minimum height=2cm,draw,rectangle,fit=(imc) (act2) (start2) (end2)](p2){};
	    \node[rotate=90,draw,rectangle,left=0.2cm of p2,xshift=1cm,yshift=-\pgflinewidth*4,minimum width=2cm] (p2l){\tiny Participant 2};
	        
	   \draw[-{Stealth[open,inset=0pt]},dashed] (imt) -- (imc); 
	   \node[draw,circle,minimum size=0.1cm,inner sep=0pt, outer sep=0pt] at (imt.south) {};
	   
	   \node[draw,cloud,fit=(b) (p2) (p2l) (p), aspect=1.6,cloud puffs = 16,minimum width=10cm,minimum height=9cm] (cloud) {};
	   
	   
	   	\node[rectangle,draw,minimum width= 3cm,minimum height=1.5cm,below=0.75 of cloud,xshift=-1.5cm](sc){Smart contract};
	    \node[rectangle,draw,minimum width= 3cm,minimum height=1.5cm,right=0cm of sc,xshift=-\pgflinewidth,align=center](c){hash(state)\\encrypt(state)};
	    \draw[-{Stealth[inset=0pt]},dashed] (c.north) +(0.5,-0.3) -- (cloud);
	    \node[below=0.1cm of c,xshift=0.6cm] (bc){Blockchain};
	    \node[draw,rectangle,fit=(c) (sc) (bc),minimum width=7cm,minimum height=2.5cm]{};
	    
	    \node[draw,semicircle,below=2.25cm of bc,minimum size=0.5cm,inner sep=0pt, outer sep=0pt,xshift=-7cm] (p1b){};
	    \node[draw,circle,below=of bc,minimum size=0.5cm,inner sep=0pt, outer sep=0pt,above=0cm of p1b] (p1h){};
	    \node[below=0.5cm of p1h]{Participant 1};
	    
	    \node[draw,semicircle,below=2.25cm of bc,minimum size=0.5cm,inner sep=0pt, outer sep=0pt,xshift=2cm] (p2b){};
	    \node[draw,circle,below=of bc,minimum size=0.5cm,inner sep=0pt, outer sep=0pt,above=0cm of p2b] (p2h){};
	    \node[below=0.5cm of p2h]{Participant 2};
	    
	    \node[right=2.8125 cm of p1b] (msg) {\huge\faEnvelope[regular]};
	    \node[below=0.25cm of msg,align=center]{DB,IPFS\\Email,IM,...};
	    
	    \draw[-{Stealth[inset=0pt]}] (p1b) to node[below,draw,circle,yshift=-0.1cm] {1.} (msg);
	    \draw[-{Stealth[inset=0pt]}] (msg) to (p2b);
	    
	    \draw[->,bend angle=25, bend left] (p1h) to node[right,align=right,yshift=-0.6cm]{update: hash(state)\\encrypt(state)\\ prove: "I'm next" \\Commit to hash(M)} node[above,draw,circle,yshift=0.45cm]{2.} (sc);
	    \draw[->,bend angle=25, bend left] (c) to node[left,align=right,yshift=-0.4cm]{Check Message M} node[above,draw,circle,xshift=0.4cm]{3.}  (p2h);
    %\node[draw,cloud,fit=(a) (b)] {};
    \end{tikzpicture}
    \caption{Overview of the zkWF protocol}
    \label{fig:basic_update}
\end{figure}


==> content/tikz-figure/smartcontract.tex <==
\begin{figure}[H]
	\centering
	\begin{tikzpicture}[font=\sffamily,line width=0.03cm]
	  \node[text centered,text width = 0.4\textwidth, text depth = 2.3 cm,
    draw,anchor=north] (sc) {Smart-contract};
        \node [above=of sc,yshift=-2.3cm,xshift=-1.15cm] (hcurr) {$\hcurr$};
		\node [right=of hcurr,xshift=-0.55cm] (Scurr){$\Ccurr$};
		\node [below=of hcurr,xshift=0.0cm,yshift=0.6cm] (sig) {$\Scurr$};
		\node[draw,dotted,fit=(Scurr) (hcurr) (sig)] {};
		\node [below=2 cm of sc] (parts) {};
		
		\node [left=of parts,xshift=1cm] (part1) {participant 1};
		\node [right=of parts,xshift=-1cm] (part2) {participant 2};
		
		\draw[<-] (sc.south -| part1) -- (part1);
		\node[above=of part1,xshift=0.5cm,yshift=0.2cm] (hash1) {$\hnew$,};
		\node[below=of hash1,yshift=1.2cm] (sig) {$\Snew$,};
		\node[below=of sig,yshift=1.2cm] (enc) {$\Cnew$,};
		\node[below=of enc,yshift=1.2cm,xshift=0.1cm] (proof) {$\proof$};
	\end{tikzpicture}
	\caption{Architecture design of the smart-contract}
	\label{fig:sc_design}
\end{figure}

==> content/tikz-figure/zkwf_program_design.tex <==
%\begin{figure}[H]
\begin{figure}
	\centering
	\begin{tikzpicture}[font=\sffamily,line width=0.03cm, scale=0.9,every node/.style={scale=0.9}]
	    \node[mybox,minimum width=6.4cm] (chk_hsh){ Checking the hash};
	    \node[mybox,below=0.0cm of chk_hsh,yshift=\pgflinewidth,minimum width=6.4cm] (chk_valid){Checking vector update validity};
	    \node[mybox,below=0cm of chk_valid,yshift=\pgflinewidth,minimum width=6.4cm] (chk_auth){ Authorization};
	    \node[below=0.075cm of chk_auth,xshift=2cm] (c_text){\large{zkWF program}};
		\node[
		rectangle,
		draw,
		minimum width= 7.5cm,
		minimum height=3.5cm,
		fit=(chk_hsh) (chk_valid) (chk_auth)] (comp) {};
		\node [above=1.5cm of comp,xshift=-1.0cm] (inputcenter) {};
		\node [left=0.75cm of inputcenter] (public) {Public inputs};
		\node [right=0.75cm of inputcenter] (private) {Private inputs};
		%Public Inputs
		\node [yshift=2.5cm,xshift=1.4cm] at (comp -| public)  (publiccenter){};
		\node [left=of publiccenter] (hcurr) {$\hcurr$};
		\node [right=of hcurr,xshift=-1.15cm] (Scurr){$\Snew$};
		\draw[<-] (comp.north -| Scurr) -- (Scurr);
		\draw[<-] (comp.north -| hcurr) -- (hcurr);
		\node[draw,dotted,fit=(Scurr) (hcurr) (public)] {};
		% Private inputs
		\node [yshift=2.5cm,,xshift=-0.4cm] at (comp -| private)  (privatecenter) {};
		 \node [left=of privatecenter] (scurr) {$\scurr$};
		 \node [right=of scurr,xshift=-1.15cm] (rcurr) {$\rcurr$};
		 \node [right=of rcurr,xshift=-1.15cm] (snew) {$\snew$};
		 \node [right=of snew,xshift=-1.15cm] (rnew) {$\rnew$};
		 \node [right=of rnew,xshift=-1.15cm] (pk) {$\pk$};
		 \node [right=of pk,xshift=-1cm] (sk) {$\sk$};
		 \draw[<-] (comp.north -| scurr) -- (scurr);
		 \draw[<-] (comp.north -| rcurr) -- (rcurr);
		 \draw[<-] (comp.north -| snew) -- (snew);
		 \draw[<-] (comp.north -| rnew) -- (rnew);
		 \draw[<-] (comp.north -| pk) -- (pk);
		 \draw[<-] (comp.north -| sk) -- (sk);
		\node[draw,dotted,fit=(pk) (sk) (rnew) (scurr) (private),minimum width=5.85cm] {};
		 % Output
		 \node [below=of comp,yshift=0.5cm] (hnew) {$\hnew=\textit{hash}(\snew|| \rnew )$};
		 \node [below=0.5cm of hnew,yshift=0.7cm] (outputs) {Outputs};
		 \draw[->] (comp.south -| hnew) -- (hnew);
		 \node[draw,dotted,fit=(outputs) (hnew),minimum width=4.5cm] {};
	\end{tikzpicture}
	\caption{The basic computation model of zkWF programs}
	\label{fig:zkwfProgram}
\end{figure}
